Blended-NeRF: Zero-Shot Object Generation and Blending in Existing Neural Radiance Fields

Editing a local region or a specific object in a 3D scene represented by a NeRF or consistently blending a new realistic object into the scene is challenging, mainly due to the implicit nature of the scene representation. We present Blended-NeRF, a robust and flexible framework for editing a specific region of interest in an existing NeRF scene, based on text prompts, along with a 3D ROI box. Our method leverages a pretrained language-image model to steer the synthesis towards a user-provided text prompt, along with a 3D MLP model initialized on an existing NeRF scene to generate the object and blend it into a specified region in the original scene. We allow local editing by localizing a 3D ROI box in the input scene, and blend the content synthesized inside the ROI with the existing scene using a novel volumetric blending technique. To obtain natural looking and view-consistent results, we leverage existing and new geometric priors and 3D augmentations for improving the visual fidelity of the final result. We test our framework both qualitatively and quantitatively on a variety of real 3D scenes and text prompts, demonstrating realistic multi-view consistent results with much flexibility and diversity compared to the baselines. Finally, we show the applicability of our framework for several 3D editing applications, including adding new objects to a scene, removing/replacing/altering existing objects, and texture conversion.

==> sections/figures.tex <==
% \begin{figure*}[p]
%     \centering
%     \setlength{\tabcolsep}{0.5pt}
%     \renewcommand{\arraystretch}{0.5}
%     \setlength{\ww}{0.4\columnwidth}
  
%     \begin{tabular}{ccccc}        
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/rose0.pdf} &
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/brocoli0.pdf} &
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/fire_hydrent0.pdf}&
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/snowboard0.pdf}&
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/zebra0.pdf}\\
        
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/rose1.pdf} &
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/brocoli1.pdf} &
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/fire_hydrent1.pdf}&
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/snowboard1.pdf}&
%         \includegraphics[width=\ww,frame]{figures/new_object_insertion/zebra1.pdf}\\
		
% 		\scriptsize{"bouguet of wilted red roses on a table."} & 
% 		\scriptsize{"broccoli laying on a plastic board."} & 
%             \scriptsize{"red and blue fire hydrant."} &
%             \scriptsize{"snowboard standing in a snow bank."} &
% 		\scriptsize{"a zebra eating grass on the ground."} \\
%     \end{tabular}
%     \caption{\textbf{Object Insertion.} Insertion of new objects from COCO dataset \cite{lin2014microsoftcoco} into an empty region in fern llff scene. Each column shows two views of the same edited scene \cite{mildenhall2019llff}.} \label{fig:coco_object_insertion}
%     %\vspace{-1mm}
% \end{figure*}


% \begin{figure*}[p]
%     \centering
%     \setlength{\tabcolsep}{0.5pt}
%     \renewcommand{\arraystretch}{0.5}
%     \setlength{\ww}{0.65\columnwidth}
  
%     \begin{tabular}{cc}        
%         \includegraphics[width=\ww,frame]{figures/ship/ship_dunes_view25.pdf}&
%         % \makebox[0pt][r]{
%         % \includegraphics[width=0.2\columnwidth,frame]{figures/ship/ship_originl_view25.pdf}}&
%         \includegraphics[width=\ww,frame]{figures/ship/ship_ice_view25.pdf}
%         \hspace{0.9cm}\makebox[0pt][b]{
%         \includegraphics[width=0.25\columnwidth,frame]{figures/ship/ship_originl_view25.pdf}}\\
        
%         \includegraphics[width=\ww,frame]{figures/ship/ship_dunes_view35.pdf}&
%         \includegraphics[width=\ww,frame]{figures/ship/ship_ice_view35.pdf}         
%         \hspace{0.9cm}\makebox[0pt][b]{
%         \includegraphics[width=0.25\columnwidth,frame]{figures/ship/ship_originl_view35.pdf}}\\
		
% 	\scriptsize{"A DLSR photo of dunes of sand."} & 
% 	\scriptsize{"A DLSR photo of ice and snow."} \\
%     \end{tabular}
    
%     \caption{\textbf{Large object replacement.} Here we preform object replacement to the blender ship scene by localizing the ROI box to include the sea and the bottom of the ship and training our model to steer the edit towards the given text prompts.} \label{fig:blender_ship}
%     %\vspace{-1mm}
% \end{figure*}

% \begin{figure*}[p]
%     \centering
%     \setlength{\tabcolsep}{0.5pt}
%     \renewcommand{\arraystretch}{0.5}
%     \setlength{\ww}{0.40\columnwidth}
  
%     \begin{tabular}{ccccc}        
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/original_pinecone_009.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/burning_pinecone_009.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/ice_pinecone_009.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/gold_pinecone_009.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/wool_pinecone_009.pdf} \\
        
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/original_pinecone_011.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/burning_pinecone_011.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/ice_pinecone_011.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/gold_pinecone_011.pdf} &
%         \includegraphics[width=\ww,frame]{figures/pinecone_texture/wool_pinecone_011.pdf} \\
		
% 		\scriptsize{Original Scene.} & 
% 		\scriptsize{"Burning pinecone".} & 
% 		\scriptsize{"Iced pinecone".} &
%             \scriptsize{"Golden pinecone".} &
%             \scriptsize{"Pinecone made of pink wool".} \\
%     \end{tabular}
    
%     \caption{\textbf{Texture Editing.} We can change only the texture of an object by freezing the layers responsible for the density and training only the layers that impact the color of the scene. To get a smooth blending, we utilize \cref{distance_blending} to blend the scene inside and outside the ROI.} \label{fig:pinecone_texture}
%     %\vspace{1mm}
% \end{figure*}


% \begin{figure*}[p]
%     \centering
%     \setlength{\tabcolsep}{0.5pt}
%     \renewcommand{\arraystretch}{0.5}
%     \setlength{\ww}{0.4\columnwidth}
  
%     \begin{tabular}{ccc}        
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_original005.pdf} &
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_original_006.pdf} &
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_original_013.pdf} \\
        
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_edit_005.pdf} &
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_edit_006.pdf} &
%         \includegraphics[width=\ww,frame]{figures/vasedeck/vase_edit_013.pdf} \\
		
%     \end{tabular}
%     \caption{\textbf{Object Insertion in vasedeck 360 scene.} We used the text: "a photo of a purple, white and blue flowers petals on the ground" and \cref{distance_blending} with $\alpha=3.5$ to generate the edit.} \label{fig:vasedeck_flower_petals}
%     %\vspace{-1mm}
% \end{figure*}


% \begin{figure*}[p]
%     \centering
%     \setlength{\tabcolsep}{0.5pt}
%     \renewcommand{\arraystretch}{0.5}
%     \setlength{\ww}{0.4\columnwidth}
  
%     \begin{tabular}{cc}        
%         \includegraphics[width=\ww,frame]{figures/blending_examples/banans_sum_in_active0.pdf} &
%         \includegraphics[width=\ww,frame]{figures/blending_examples/mashrooms_sum_in_active0.pdf} \\
        
%         \includegraphics[width=\ww,frame]{figures/blending_examples/banans_sum_in_active1.pdf} &
%         \includegraphics[width=\ww,frame]{figures/blending_examples/mashrooms_sum_in_active1.pdf} \\
		
%             \scriptsize{"a few green and yellow bananas".} &
%             \scriptsize{"clusters of different types of mushrooms".} \\
%     \end{tabular}
%     \caption{\textbf{Blending Densities Inside Activation.} We demonstrate our suggested blending procedure for blending the original and synthesized objects inside the ROI in llff fern scene \cite{mildenhall2019llff} using \cref{sigma_in_eqn} for summing the densities.} \label{fig:fern_blending}
%     %\vspace{-1mm}
% \end{figure*}

